On the absence of the electrostriction force in dilute clouds of cold atoms

The momentum of light in a medium and the mechanisms of momentum transfer between light and dielectrics have long been the topic of controversies and confusion. We discuss here the problem of momentum transfers that follow the refraction of light by dilute, inhomogeneous ensembles of ultra-cold atoms. We show experimentally and theoretically that the refraction of light rays by a dilute gas does not entail momentum transfers to first order in the light-atom coupling coefficient, in contradiction with the work reported in Matzliah et al. Phys. Rev. Lett. 119, 189902 (2017).

==> comment_on_ES_revised.tex <==
 reprint,
 amsmath,amssymb,
 aps,nofootinbib
]{revtex4-2}

\usepackage{graphicx}
\usepackage{dcolumn}
\usepackage{bm}
\usepackage{mathtools}
\usepackage{physics}
\usepackage{amsmath}




\newcommand{\gguide}{{\it Preparing graphics for IOP journals}}
\newcommand{\expect}[1]{\left\langle#1\right\rangle}
\newcommand{\com}[2]{\left[#1,#2\right]}
\newcommand{\fig}[1]{\mbox{Fig. #1}}
\newcommand{\ppsi}{\left\vert \psi \right\rangle}
\newcommand{\hilight}[1]{\colorbox{yellow}{#1}}
\newcommand{\pd}[2]{\ensuremath{\frac{\partial #1}{\partial #2}}}
\newcommand{\ppd}[2]{\ensuremath{\frac{\partial^2 #1}{\partial #2^2}}}
\newcommand{\fracm}[2]{\ensuremath{\ \frac{\mbox{#1}}{\mbox{#2}}}}
\newcommand{\na}{\ensuremath{\mathbf\nabla}}
\newcommand{\bitem}[1]{\item {\bf #1}}
\newcommand{\eg}{\emph{e.g.} }
\newcommand{\kg}{\mbox{ kg}}
\newcommand{\mum}{$\rm\mu m$ }
\newcommand{\m}{\mbox{ m }}
\newcommand{\cm}{\mbox{ cm }}
\newcommand{\mm}{\mbox{ mm }}
\newcommand{\km}{\mbox{ km }}
\newcommand{\nm}{\mbox{ nm }}
\newcommand{\ms}{\mbox{ ms }}
\newcommand{\se}{\mbox{ sec}}
\newcommand{\erg}{\mbox{ erg}}
\newcommand{\Hz}{\mbox{ Hz }}
\newcommand{\kHz}{\mbox{ kHz }}
\newcommand{\MHz}{\mbox{ MHz }}
\newcommand{\GHz}{\mbox{ GHz }}
\newcommand{\THz}{\mbox{ THz}}
\newcommand{\mW}{\mbox{ mW }}
\newcommand{\W}{\mbox{ W }}
\newcommand{\eV}{\mbox{ eV}}
\newcommand{\keV}{\mbox{ keV}}
\newcommand{\MeV}{\mbox{ MeV}}
\newcommand{\GeV}{\mbox{ GeV}}
\newcommand{\TeV}{\mbox{ TeV}}
\newcommand{\K}{\mbox{ K }}	
\newcommand{\nK}{\mbox{ nK }}
\newcommand{\Er}{\mbox{ $\rm E_r$}}
\newcommand{\muK}{ $\rm\mu K$}
\newcommand{\h}{$\hbar$}
\newcommand{\hk}{$\rm\hbar k$ }
\newcommand{\D}{\mathcal{D}}
\newcommand{\Ha}{\mathcal{H}}
\newcommand{\der}[2]{\ensuremath{\frac{d #1}{d #2}}}
\newcommand{\dsq}[2]{\ensuremath{\frac{d^2 #1}{d #2^2}}}
\newcommand{\sps}{\mbox{ }}
\newcommand{\Rb}{\ensuremath{^{87}}Rb}
\newcommand{\tp}{\ensuremath{\tau}_p }

\newcommand{\Psidt}{\Psi(\mathbf{r},t)}
\newcommand{\Psid}{\Psi(\mathbf{r})}
\newcommand{\Psidts}{\Psi^\ast(\mathbf{r},t)}
\newcommand{\Psids}{\Psi^\ast(\mathbf{r})}
\newcommand{\Psis}{\Psi^\ast}
\newcommand{\eq}[2]{\begin{equation}#1\label{#2}\end{equation}}
\newcommand{\eqal}[2]{\begin{align}#1\label{#2}\end{align}}
\newcommand{\pard}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\pardd}[2]{\frac{\partial^2 #1}{\partial #2^2}}
\newcommand{\rv}{\mathbf{r}}
\newcommand{\abso}[1]{\left| #1 \right|}
\newcommand{\nabv}{\mathbf{\nabla}}
\newcommand{\Hop}{\hat{\mathrm{H}}}

\newcommand{\amk}{\hat{a}_{-\mathbf{k}}}
\newcommand{\amkd}{\hat{a}_{-\mathbf{k}}^\dagger}
\newcommand{\bki}[1]{\hat{b}_{\mathbf{k_#1}}}
\newcommand{\bkid}[1]{\hat{b}_{\mathbf{k_#1}}^\dagger}
\newcommand{\bk}{\hat{b}_{\mathbf{k}}}
\newcommand{\bmk}{\hat{b}_{-\mathbf{k}}}
\newcommand{\bkd}{\hat{b}_{\mathbf{k}}^\dagger}
\newcommand{\bmkd}{\hat{b}_{-\mathbf{k}}^\dagger}

\newcommand{\bop}[1]{\hat{b}_{#1}}
\newcommand{\bopd}[1]{\hat{b}_{#1}^\dagger}
\newcommand{\kv}{\mathbf{k}}
\newcommand{\qv}{\mathbf{q}}

\newcommand{\psopx}{\hat{\Psi}\left(x\right)}
\newcommand{\psopdx}{\hat{\Psi}^\dagger\left(x\right)}
\newcommand{\kin}{-\frac{\hbar^2}{2m}\nabv^2}
\newcommand{\aip}{\hat{a}_{i+1}}
\newcommand{\ai}{\hat{a}_i}
\newcommand{\aid}{\hat{a}_i^\dagger}
\newcommand{\aj}{\hat{a}_j}
\newcommand{\ajd}{\hat{a}_j^\dagger}
\newcommand{\aop}{\hat{a}}
\newcommand{\aopd}{\hat{a}^\dagger}

\newcommand{\cop}[1]{\hat{c}_{#1}}
\newcommand{\copd}[1]{\hat{c}^\dagger_{#1}}


\newcommand{\dop}{\hat{\vb{d}}}
\newcommand{\dopd}{\hat{d}^\dagger}
\newcommand{\Jops}{\hat{J}^2}
\newcommand{\Jopsd}{\hat{J}^2^\dagger}

\newcommand{\sigx}{\hat{\sigma}_x}
\newcommand{\sigy}{\hat{\sigma}_y}
\newcommand{\sigz}{\hat{\sigma}_z}
\newcommand{\sigp}{\hat{\sigma}_+}
\newcommand{\sigm}{\hat{\sigma}_-}


\newcommand{\ie}{\textit{i.e. }}

\begin{document}

\preprint{APS/123-QED}

\title{Comment on Phys.Rev.Lett. 119, 163201 (2017)}


\author{authors}
\affiliation{Department of Physics of Complex Systems, Weizmann Institute of Science, Rehovot 761001, Israel}

\date{\today}

\begin{abstract}

\end{abstract}


\maketitle
% \def\thefootnote{$\dagger$}\footnotetext{Corresponding author : nir.davidson@weizmann.ac.il}

In this comment, we report on new developments concerning electrostriction, a force predicted and measured by \textit{Matzliah et. al} in \cite{NH}. In a few words, electrostriction was thought to manifest as a consequence of momentum conservation following the refraction of light by an inhomogeneous atomic ensemble. The new theoretical and experimental efforts reviewed in this comment point towards the non-existence of this force in the form that was previously thought-of. 
\newline\indent
The expression of the force reported in equation (1) of \cite{NH} was derived in the limit of a dilute dielectric material, and appears to be to first order in the single-atom polarizability. This result is in contradiction with well-established theories on the force density experienced by dielectrics in the presence of electromagnetic radiation \cite{ll,milonni2010,brevik1978}. In the limit of non-magnetic dielectric materials where pressure gradients are insignificant, and when one is interested in forces averaged over an optical cycle, the correct expression for the force density is given by
\eq{
\vb f = -\frac{\epsilon_0}{2}\vb E^2\grad{\epsilon}\ +\frac{\epsilon_0}{2}\pmb\nabla\left(\pard{\epsilon}{n^*}n^*\vb E^2\right),
}{eq:ll}
where $\epsilon_0$ is the vacuum permittivity, $\epsilon$ is the relative permittivity of the material, $n^*$ is the ensemble density and $\vb E$ is the electric field amplitude. In \cite{NH}, the authors omitted both the longitudinal component in the first term of equation (\ref{eq:ll}) and the second term altogether. In the case of plane-wave irradiation far from atomic resonances and in the limit of dilute gases \ie when $\epsilon\propto n^*$, the two terms compensate one-another and the force density vanishes. This is in contradiction with every experimental results published in \cite{NH}. 
\newline\indent
In figure 4 of \cite{NH}, \textit{Matzliah et. al} report on variations of the ensemble's aspect ratio after time-of-flight, $AR$, as a function of various experimental parameters such as the laser's detuning and intensity. Changes in $AR^2-1$ were thought to be the result of the transverse force they wrongly predicted. Reproducing the experiment in a different experimental setup and in a well-controlled setting, we measured no variations of $AR^2-1$, in agreement with equation (\ref{eq:ll}), taken in the appropriate limits. We used a thermal ensemble of \Rb\ containing approximately $5\times10^5$ atoms at a temperature of 400nK, in a far-off-resonance optical dipole trap with oscillation frequencies of about $90\rm Hz$. We set the electrostriction beam detuning, $\Delta$, between $-30\rm GHz$ and $-100\rm GHz$ with respect to the $F=1$ to $F'=2$ transition of the $D_2$ line of \Rb. We measure the maximum on-atom intensity to be $4.5\times10^4\rm W.m^{-2}$. We release the atoms from the confining potential and immediately pulse the electrostriction beam for $400\rm\mu s$, and finally measure the cloud's aspect ratio after $20\rm ms$ of time-of-flight. In figure \ref{fig:noes}, we show the comparison between our new experiment and the theory published in \cite{NH} for different detunings and intensities. At a detuning of $-50\rm GHz$ and at maximal intensity, the theory prediction is larger than our measurement by more than a thousand standard deviations.
\begin{figure}[h]
    \centering
    \includegraphics[width = \columnwidth]{no_es_alt.png}
    \caption{Comparison between experiment (circular markers) and theory (dashed lines) showing the absence of electrostriction as described by the theory of \cite{NH}. The aspect ratio, $AR$, was measured after 20ms of time-of-flight. Each data point was obtained by averaging 30 experimental runs and the data was collected in a random order. Error-bars correspond to the standard deviation of the data-spread. The maximum intensity is set to be $4.5\times10^4\rm W.m^{-2}$.}
    \label{fig:noes}
\end{figure}
\newline\indent
In addition to new experimental results, we have evidence that the non-unity aspect ratios measured in \cite{NH} were the result of a dipole force due to residual imperfections on the beam used. Every recent theoretical and experimental developments point to the absence of an electrostriction force in the regime studied in \cite{NH}.
\section*{Acknowledgements}
The authors acknowledge fruitful discussions with Ulf Leonhardt, Ephraim Shahmoon and Amruta Gadge. 
\bibliography{biblio}

\end{document}

